A General Theory for the Evolution of Application Models -- Full version

In this article we focus on evolving information systems. First a delimitation of the concept of evolution is provided, resulting in a first attempt to a general theory for such evolutions. The theory makes a distinction between the underlying information structure at the conceptual level, its evolution on the one hand, and the description and semantics of operations on the information structure and its population on the other hand. Main issues within this theory are object typing, type relatedness and identification of objects. In terms of these concepts, we propose some axioms on the well-formedness of evolution. In this general theory, the underlying data model is a parameter, making the theory applicable for a wide range of modelling techniques, including object-role modelling and object oriented techniques.

==> eu02beha.tex <==
\unitlength=0.70\unitlength
\begin{Picture}{320}{135}{0}
  \put(0,50){
  \SetBoxDims{19}{29}{0}
  \state{ 15}{ 25}{}
  \SetBoxDims{15}{15}{0}
  \state{ 17}{ 55}{}
  \thicklines
  \lseg{  15}{ 45}{-1}{ 1}{15}
  \lseg{  34}{ 45}{ 1}{ 1}{15}
  \lseg{  18}{ 26}{-1}{-2}{10}
  \lseg{  30}{ 26}{ 1}{-2}{10}
  }
  \SetBoxDims{80}{30}{4}

  \CalcLines
  \environment{100}{100}{$H_{uod}$}
  \DottedVect(35,115)(100,115)
  \Text{66}{119}{observing}{b}

  \Vect(35,110)(140,30)
  \Text{87}{73}{formulating}{l}
  \state{100}{  0}{$E$}

  \DVect(180,15)(240,15)
  \Text{210}{17}{$\Behaves$}{b}
  \state{240}{  0}{$H_{is}$}

  \DVect(180,115)(285,30)
  \Text{233}{73}{validation}{l}
  \PutLines
\end{Picture}


==> eu02evol.tex <==
\begin{Picture}{50}{100}{0}


\def\Dot(#1,#2){\SetTextSize{1} \Text{#1}{#2}{$\bullet$}{c}}

\Dot( 5,20)
\Dot(15,40)
\Dot(25,30)
\Dot(35,40)
\Dot(45,35)
\DottedLine( 5,20)(15,40)(25,30)(35,40)(45,35)

\Dot( 5,70)
\Dot(15,60)
\Dot(25,56)
\Dot(35,56)
\Dot(45,50)
\DottedLine( 5,70)(15,60)(25,56)(35,56)(45,50)

\Dot( 5,85)
\Dot(15,75)
\Dot(25,81)
\Dot(35,80)
\Dot(45,85)
\DottedLine( 5,85)(15,75)(25,81)(35,80)(45,85)

\DrawLine( 5,0)( 5,100)
\DrawLine(15,0)(15,100)
\DrawLine(25,0)(25,100)
\DrawLine(35,0)(35,100)
\DrawLine(45,0)(45,100)

\Vect(60,0)(90,0)
\Text{75}{ 5}{\em time}{b}

\end{Picture}

==> eu02evsh.tex <==
\begin{Picture}{90}{100}{0}

\CalcLines
\def\SnapShot#1{
   \put(#1,0){\DrawLine(10,10)(0,0)(0,50)(50,100)(50,90)}
}

\SnapShot{ 0}
\SnapShot{10}
\SnapShot{20}
\SnapShot{30}
\SnapShot{40} \DrawLine(40,0)(90,50)(90,100)

\def\Dot(#1,#2){\SetTextSize{1} \Text{#1}{#2}{$\bullet$}{c}}

\Dot( 5,20)
\Dot(15,40)
\Dot(25,30)
\Dot(35,40)
\Dot(45,35)
\DottedLine( 5,20)(15,40)(25,30)(35,40)(45,35)

\Dot(25,70)
\Dot(27,60)
\Dot(32,56)
\Dot(43,56)
\Dot(55,50)
\DottedLine(25,70)(27,60)(32,56)(43,56)(55,50)

\Dot(40,85)
\Dot(41,75)
\Dot(55,81)
\Dot(65,80)
\Dot(80,85)
\DottedLine(40,85)(41,75)(55,81)(65,80)(80,85)

\Vect(60,0)(90,0)
\Text{75}{ 5}{\em time}{b}

\end{Picture}


==> eu02lpl1.tex <==
\unitlength=1.1\unitlength
\begin{Picture}{180}{100}{0}
  \SetBoxDims{40}{40}{2}
  \Entity{  0}{ 60}{LP\\[3pt] \# Title~ \\ \# Artist} 
  \Entity{140}{ 60}{Song\\[3pt] \# Title~~~ \\ \# Author}
  \Entity{140}{  0}{Frequency\\[3pt] \# Times}

  \SetBoxDims{60}{40}{2}
  \Relation{ 60}{ 60}{Recording}
  \Relation{ 60}{  0}{Lending-\\frequency}

  \DrawLine( 20, 60)( 60, 20)
  \DrawLine(120, 20)(140, 20)
  \DrawLine( 40, 80)( 60, 80)
  \DrawLine(120, 80)(140, 80)
\end{Picture}


==> eu02lpl2.tex <==
\unitlength=1.1\unitlength
\begin{Picture}{180}{180}{0}
\put(0,80){
  \SetBoxDims{40}{40}{2}
  \Entity{  0}{ 60}{Medium\\[3pt] \# Title~ \\ \# Artist} 
  \Entity{140}{ 60}{Song\\[3pt] \# Title~~~ \\ \# Author}
  \Entity{ 70}{-10}{CD}
  \Entity{  0}{-80}{LP}
  \Entity{140}{-80}{Frequency\\[3pt] \# Times}
  
  \Relation{  0}{-10}{~\\Medium-\\type}
  \SetBoxDims{60}{40}{2}
  \Relation{ 60}{ 60}{Recording} 
  \Relation{ 60}{-80}{Lending-\\frequency}
  
  \DrawLine( 20, 60)( 20, 30)
  \DrawLine( 15, 55)( 25, 55)
  \DrawLine( 20,-10)( 20,-40)
  \DrawLine( 40, 10)( 70, 10)

  \DrawLine( 40, 80)( 60, 80)
  \DrawLine(120, 80)(140, 80)

  \DrawLine( 40,-60)( 60,-60)
  \DrawLine(120,-60)(140,-60)
}
\end{Picture}


==> eu02lplt.tex <==
\unitlength=1.1\unitlength
\begin{Picture}{180}{160}{0}
\put(0,60){
  \SetBoxDims{40}{40}{2}
  \Entity{  0}{ 60}{LP\\[3pt] \# Title~ \\ \# Artist} 
  \Entity{140}{ 60}{Song\\[3pt] \# Title~~~ \\ \# Author}
  \Entity{ 70}{-60}{\large $\Time_{\!\!\it interval}$}

  \SetBoxDims{60}{40}{2}
  \Entity{ 60}{ 60}{}
  \Relation{ 60}{ 60}{Recording}

  \SetBoxDims{40}{40}{2}
  \Relation{ 70}{ 0}{Object-\\type}

  \DrawLine( 20, 60)( 70, 20)
  \DrawLine(110, 20)(160, 60)
  \DrawLine( 90, 40)( 90, 60)
  \DrawLine( 40, 80)( 60, 80)
  \DrawLine(120, 80)(140, 80)
  \DrawLine( 90,  0)( 90,-20)
  \DrawLine( 85,-15)( 95,-15)
}
\end{Picture}


==> eu02mohi.tex <==
\begin{Picture}{155}{140}{0}
\put(-65,-110){
\SetTextSize{3}
\Text{ 75}{115}{Information\\Structure}{c}
\Text{145}{115}{Constraints}{c}
\Text{215}{115}{Population}{c}
\Text{145}{175}{World\\Model}{c}
\Text{215}{175}{Action\\Model}{c}
\Text{180}{235}{Application\\Model}{c}

\Vect(145,165)( 78,125)
\Vect(145,165)(145,120)
\Vect(145,165)(213,120)
\Vect(180,225)(147,185)
\Vect(180,225)(213,185)

\Text{ 35}{240}{Legend:}{lc}
\SetTextSize{2}
\Vect( 40,230)( 68,230)
\Text{67}{230}{= contains}{lc}
}
\end{Picture}



==> eu02snsh.tex <==
\begin{Picture}{90}{100}{0}

\CalcLines
\def\SnapShot#1{
   \put(#1,0){\DrawLine(10,10)(0,0)(0,50)(50,100)(50,90)}
}

\SnapShot{ 0}
\SnapShot{10}
\SnapShot{20}
\SnapShot{30}
\SnapShot{40} \DrawLine(40,0)(90,50)(90,100)


\def\Dot(#1,#2){\SetTextSize{1} \Text{#1}{#2}{$\bullet$}{c}}

\Dot( 5,20)
\Dot(15,40)
\Dot(25,30)
\Dot(35,40)
\Dot(45,35)

\Dot(25,70)
\Dot(27,60)
\Dot(32,56)
\Dot(43,56)
\Dot(55,50)

\Dot(40,85)
\Dot(41,75)
\Dot(55,81)
\Dot(65,80)
\Dot(80,85)

\Vect(60,0)(90,0)
\Text{75}{ 5}{\em time}{b}
\end{Picture}


==> eu03trdg.tex <==
\unitlength=2\unitlength
\begin{Picture}{50}{60}{0}

\put(-90,0){
\total{ 90}{20}
\total{115}{10}
\total{140}{20}

\total{ 90}{35}
\total{140}{35}

\total{ 90}{55}
\total{140}{55}

\SetDefaultDotGap{1}
\DottedDrawing
\thicklines
   \SampleStep{30}
   \put(114,  4){\Arc{12}{0}{360}}
   \Vect(118,  8)(117,  9)

   \Vect( 90, 20)(113, 11)
   \Vect(140, 20)(117, 11)

   \Vect( 90, 55)( 90, 36)
   \Vect(140, 55)(140, 36)
\thinlines
\SolidDrawing
 
\Text{ 86}{16}{B}{c}
\Text{115}{14}{A}{b}
\Text{144}{16}{C}{c}

\Text{ 86}{31}{D}{c}
\Text{144}{31}{E}{c}

\Text{ 86}{51}{F}{c}
\Text{144}{51}{G}{c}

\Text{115}{34}{$\TypeRel$}{c}
\DottedDrawing
   \Vect(115, 40)(115, 50)
\SolidDrawing
\Text{115}{54}{$\TypeRel$}{c}
}

\end{Picture}


==> eu03tyre.tex <==
\begin{Picture}{110}{130}{0}

\SetBoxDims{30}{30}{2}
\type{ 40}{  0}{A}
\type{  0}{ 40}{} \Text{ 30}{70}{D}{c}
\type{ 80}{ 40}{} \Text{110}{70}{E}{c}
\type{  0}{100}{F}
\type{ 80}{100}{G}

\SetBoxDims{22}{22}{2}
\type{  4}{ 44}{B}
\type{ 84}{ 44}{C}

\SetBoxDims{24}{24}{2}
\thicklines
   \DottedDrawing
       \Vect( 16, 70)(16,100)
       \Vect( 96, 70)(96,100)
   \SolidDrawing

   \Vect( 4,44)[ -45](40, 0)<32,32>[135]
   \Vect(84,42)[-135](40,-2)<32,32>[ 45]
\thinlines

\end{Picture}


==> eu04airp.tex <==
\unitlength=1.2\unitlength
\begin{Picture}{240}{150}{0}

\put(0,30){
\SetBoxDims{30}{30}{1}

\type{ 60}{  0}{Un-\\registered-\\airplane}
\type{120}{  0}{Registered-\\airplane}[0]
\type{210}{  0}{Owner\\(Name)}[180]
\type{ 90}{ 50}{Airplane\\(PL-Code)} 
\type{  0}{ 50}{Age\\(Nr)}
\type{180}{ 50}{Admission-\\code\\(Adm-Id)}[180]
\type{  0}{ 90}{Manufac-\\turer\\(Name)}[0]

\SetBoxDims{20}{20}{1}
\hfac{150}{  5}{20}{\hroles{is-owned-\\by}{of}}{}
\hunique{170}{  5}{-1}{0}{1}

\hfac{ 30}{ 55}{20}{\hroles{of}{has-as}}{}
\hunique{ 50}{ 55}{-1}{1}{1}

\hfac{120}{ 55}{20}{\hroles{received}{given-to}}{}
\hunique{140}{ 55}{-1}{0}{1}

\hfac{ 50}{ 95}{0}{\hroles{builds}{build-by}}{}
\hunique{ 50}{ 95}{-1}{0}{2}

\SetBoxDims{30}{30}{1}
\DrawLine( 30,105)( 50,105)
\DrawLine( 70,105)( 93, 50)[90]

\thicklines
   \Vect( 74, 30)(104, 50)
   \Vect(136, 30)(106, 50)
\thinlines
}

\Text{120}{10}{\SmallSize \begin{tabular}{lll}
\LISA{Registered-airplane}   & = & \LISA{Airplane received Admission-code}\\
\LISA{Unregistered-airplane} & = & \LISA{Airplane BUT-NOT Registered-airplane}
\end{tabular}}{c}

\end{Picture}


==> eu04simm.tex <==
\unitlength=1\unitlength
\begin{Picture}{290}{150}{0}

\put(0,5){
\SetBoxDims{30}{30}{5}
\type{  0}{  0}{$\UniDom$}
\type{100}{  0}{$\NLTypes_t$}
\type{160}{  0}{$\LTypes_t$}[0]
\type{260}{  0}{$\ConcrDoms$}
\type{130}{ 60}{$\OTypes_t$}
\type{  0}{100}{$\ConstrDef$}
\type{ 55}{100}{}
\type{205}{100}{}
\type{260}{100}{$\TaskDef$}

\SetBoxDims{40}{40}{5}
\type{125}{ 55}{} 
\type{ 50}{ 95}{} \Text{ 90}{135}{$\Constraints_t$}{c}
\type{200}{ 95}{} \Text{245}{135}{$\Tasks_t$}{c}

\SetBoxDims{20}{20}{5}
\hfac{ 55}{  5}{0}{}{$\HasTypes_t$}
\hunique{ 55}{  5}{1}{0}{2}
\DrawLine( 30, 15)( 55, 15)
\DrawLine( 75, 15)(125, 55)<40,40>[-135]

\hfac{190}{  5}{25}{}{$\Domain_t$}
\hunique{215}{  5}{1}{0}{1}

\hfac{ 60}{105}{0}{}{}
\hunique{ 60}{105}{1}{0}{2}
\DrawLine( 30,115)( 60,115)
\DrawLine( 80,115)(130, 60)<30,31>[100]

\hfac{210}{105}{0}{}{}
\hunique{210}{105}{1}{0}{2}
\DrawLine(260,115)(230,115)
\DrawLine(210,115)(130, 60)<30,31>[80]

\vfac{ 95}{ 65}{0}{$\TypeRel_t$}{}
\vunique{ 95}{ 65}{1}{0}{2}
\DrawLine(107, 80)(130, 60)<30,30>[160]
\DrawLine(107, 70)(130, 60)<30,30>[200]
\Text{ 97}{ 85}{*}{c}

\vfac{175}{ 65}{0}{}{$\ParentOf_t$}{}
\vunique{175}{ 65}{-1}{0}{2}
\DrawLine(181, 80)(130, 60)<30,30>[ 20]
\DrawLine(181, 70)(130, 60)<30,30>[-20]
\Text{191}{ 85}{*}{c}

\thicklines
\DottedDrawing
   \Vect(115, 30)(130, 58)<30,30>[-100]
   \Vect(175, 30)(130, 58)<30,30>[ -80]
\SolidDrawing
\thinlines
}

\end{Picture}


==> eu05evmm.tex <==
\unitlength=1.0\unitlength
\begin{Picture}{310}{290}{0}

\put(10,5){
\SetBoxDims{30}{30}{5}
\type{  0}{  0}{$\UniDom$}
\type{ 50}{  0}{}
\type{100}{  0}{$\NLTypes$}
\type{160}{  0}{$\LTypes$}
\type{210}{  0}{}
\type{260}{  0}{$\ConcrDoms$}
\type{130}{ 60}{$\OTypes$}
\type{  0}{100}{$\ConstrDef$}
\type{ 55}{100}{}
\type{205}{100}{}
\type{260}{100}{$\TaskDef$}
\type{240}{165}{$\Time$}
\Type{115}{150}{165}{60} \Text{283}{210}{$\AMH$}{c}

\SetBoxDims{40}{40}{5}
\type{  5}{245}{$\ObjEvol$}
\type{ 65}{245}{$\ConstrEvol$}
\type{125}{245}{$\TaskEvol$}
\type{185}{245}{$\PopEvol$}
\type{245}{245}{$\DomEvol$}
\type{125}{160}{$\AME$}
\type{125}{ 55}{} 
\type{ 50}{ 95}{} \Text{ 90}{135}{$\Constraints$}{c}
\type{200}{ 95}{} \Text{245}{135}{$\Tasks$}{c}

\thicklines
\CalcLines
   \Vect( 25,245)(140,210)
   \Vect( 85,245)(167,210)
   \Vect(145,245)(194,210)
   \Vect(205,245)(221,210)
   \Vect(265,245)(248,210)
\PutLines
\DottedDrawing
   \Vect( 65, 30)(-10,100)(-10,130)(125,160)<40,40>[210]
   \Vect(225, 30)(300,100)(300,130)(125,160)<40,40>[-30]
   \Vect( 70,130)(125,160)<40,40>[240]
   \Vect(220,130)(125,160)<40,40>[-60]
   \Vect(145, 90)(145,160)
   \Vect(115, 30)(130, 58)<30,30>[-100]
   \Vect(175, 30)(130, 58)<30,30>[ -80]
\SolidDrawing
\thinlines

\SetBoxDims{20}{20}{5} \SmallSize 
\hfac{ 55}{  5}{0}{}{$\HasTypes$}
\hunique{ 55}{  5}{1}{0}{2}
\DrawLine( 30, 15)( 55, 15)
\DrawLine( 75, 15)(125, 55)<40,40>[-135]
\hfac{190}{  5}{25}{}{$\Domain$}
\hunique{215}{  5}{1}{0}{2}
\NormalSize

\hfac{ 60}{105}{0}{}{}
\hunique{ 60}{105}{1}{0}{2}
\DrawLine( 30,115)( 60,115)
\DrawLine( 80,115)(130, 60)<30,31>[100]

\hfac{210}{105}{0}{}{}
\hunique{210}{105}{1}{0}{2}
\DrawLine(260,115)(230,115)
\DrawLine(210,115)(130, 60)<30,31>[80]

\hfac{165}{170}{28}{\SF{AME-Evol}}{}
\hunique{190}{170}{-1}{0}{2}

\vfac{ 95}{ 65}{0}{$\TypeRel$}{}
\vunique{ 95}{ 65}{1}{0}{2}
\DrawLine(107, 80)(130, 60)<30,30>[160]
\DrawLine(107, 70)(130, 60)<30,30>[200]

\vfac{175}{ 65}{0}{}{$\ParentOf$}{}
\vunique{175}{ 65}{-1}{0}{2}
\DrawLine(181, 80)(130, 60)<30,30>[ 20]
\DrawLine(181, 70)(130, 60)<30,30>[-20]
}

\end{Picture}


==> fa01p01.tex <==
\begin{Picture}{240}{270}{0}
\put(-5,0){
  \SetBoxDims{50}{30}{3}

  \activ{125}{  5}{{\em \shortstack{way\\of\\support}}}
  \activ{ 75}{ 85}{{\em \shortstack{way\\of\\modelling}}}
  \activ{175}{ 85}{{\em \shortstack{way\\of\\working}}}
  \activ{125}{235}{{\em \shortstack{way\\of\\thinking}}}
  \SetBoxDims{150}{30}{3}
  \activ{ 75}{165}{{\em way of control}}

  \SetBoxDims{170}{55}{3}
  \activ{ 65}{  70}{}

  \Text{100}{ 77}{{\em product}}{}
  \Text{200}{ 77}{{\em process}}{}
  \Text{  5}{100}{{\em operational}}{l}
  \Text{  5}{180}{{\em managerial}}{l}

  \flow{135}{ 40}{-4}{ 3}{35}
  \flow{145}{ 40}{-2}{ 3}{18}
  \flow{155}{ 40}{ 2}{ 3}{18}
  \flow{165}{ 40}{ 4}{ 3}{35}

  \flow{135}{230}{-4}{-3}{35}
  \flow{145}{230}{-2}{-3}{18}
  \flow{155}{230}{ 2}{-3}{18}
  \flow{165}{230}{ 4}{-3}{35}

  \flow{125}{100}{ 1}{ 0}{50}
  \flow{175}{100}{-1}{ 0}{50}

  \flow{100}{165}{ 0}{-1}{40}
  \flow{200}{125}{ 0}{ 1}{40}
}
\end{Picture}


==> fu02lpl3.tex <==
\unitlength=1.1\unitlength
\begin{Picture}{180}{40}{0}
  \SetBoxDims{40}{40}{2}
  \put(0,-60){
  \Entity{  0}{ 60}{CD\\[3pt] \# Title~ \\ \# Artist} 
  \Entity{140}{ 60}{Song\\[3pt] \# Title~~~ \\ \# Author}

  \SetBoxDims{60}{40}{2}
  \Relation{ 60}{ 60}{\shortstack{Recording\\ \# Quality}}

  \DrawLine( 40, 80)( 60, 80)
  \DrawLine(120, 80)(140, 80)
  }
\end{Picture}


==> gu02hist.tex <==
%\footnotesize
 \begin{tabular}{lc|l|l|l}
    & \shortstack{point\\of\\time} & LP & CD & Recording \\
    \hline
    time $\downarrow$
      & $t_0$
          & object type 
          & {\em non existent}
          & relation between \LISA{LP} and \LISA{Song}  \Forc{3} \\
      & $t_1$
          & subtype     
          & subtype       
          & relation between \LISA{Medium} and \LISA{Song} \Forc{3} \\
      & $t_2$
          & {\em non existent}
          & object type
          & relation between \LISA{CD} and \LISA{Song} \Forc{3}
 \end{tabular}



==> gu03mrex.tex <==
\unitlength=1.25\unitlength
\begin{Picture}{300}{110}{0}
\put(120,-40){
  \SetBoxDims{30}{30}{1}
  \type{150}{ 40}{(Zip\\code)}[180]
  \type{  0}{ 60}{Boat\\(Regnr)}[180]
  \type{ 60}{ 60}{House}[45][-45]
  \type{150}{ 80}{(Housenr)}[180]
  \type{ 30}{120}{Product}[0]
  \type{150}{120}{Amount\\(ECU)}[180]
  \type{-30}{120}{Real\\estate}[0]
  \type{-120}{120}{Tax\\percentage\\(\%)}
  \type{-90}{ 60}{Size\\(Tons)}
 
  \thicklines
  \Vect(0,135)(30,135) 
  \DottedVect(14,90)(44,120)
  \DottedVect(76,90)(46,120)
  \thinlines

  \SetBoxDims{20}{20}{1}
  \hfac{110}{ 45}{0}{}{\hroles{has}{is of}}
  \hunique{110}{ 45}{1}{0}{1}
  \DrawLine( 60, 60)<30,30>[-45](110, 55)
  \DrawLine(130, 55)(150, 55)

  \hfac{-60}{ 65}{20}{}{\hroles{of}{has}}
  \hunique{-40}{ 65}{1}{1}{1}

  \hfac{-90}{125}{20}{}{\hroles{of}{has}}
  \hunique{-70}{125}{1}{1}{1}

  \hfac{110}{ 85}{0}{\hroles{has}{is of}}{}
  \hunique{110}{ 85}{-1}{0}{1}
  \DrawLine( 60, 60)<30,30>[45](110, 95)
  \DrawLine(130, 95)(150, 95)

  \hfac{110}{125}{0}{}{\hroles{has price}{is price\\of}}
  \hunique{110}{125}{1}{0}{1}
  \DrawLine( 30,120)<30,30>[0](110,135)
  \DrawLine(130,135)(150,135)

  \Constraint{135}{75}(\Unique)
  \DottedLine(135, 70)(125, 58)
  \DottedLine(135, 80)(125, 90)
}
\end{Picture}


==> gu03rtdg.tex <==
\unitlength=2\unitlength
\begin{Picture}{70}{70}{0}
\put(-10,-10){
   \SetBoxDims{30}{30}{2}
   \total{20}{20}
   \total{70}{20}
   \total{20}{70}
   \total{70}{70}

   \SetDefaultDotGap{1}
   \DottedDrawing \thicklines
      \Vect( 20, 68)( 20, 22)
      \Vect( 20, 68)( 68, 22)
      \Vect( 70, 68)( 22, 22)
      \Vect( 70, 68)( 70, 22)
      \SampleStep{30}
      \put(17,14){\Arc{12}{0}{360}}
      \Vect( 22, 16)(21, 18)
      \put(73,14){\Arc{12}{0}{360}}
      \Vect( 68, 17)(69, 18)
   \SolidDrawing \thinlines

   \Text{16}{25}{Boat}{r}
   \Text{74}{25}{House}{l}
   \Text{16}{74}{Real\\estate}{r}
   \Text{74}{74}{Product}{l}
}
\end{Picture}


==> gu06.tex <==
\section{Evolution of Application Models}
\SLabel{section}{AMEvolv}

As stated before, the evolution of an application model is described
by the evolution of its elements.
The set $\AME$ was introduced as the set of all evolvable elements of an
application model.
Its formal definition in terms of components of $\AppModUniverse$ is:
\begin{definition} Application model elements:
   \Intro{\AME}{application model elements}
   \[
      \AME = \OTypes \union \Constraints \union \Tasks \union
             \HasTypes \union \Domain
   \]
\end{definition}
An \keyword{application model element evolution} was defined as a partial function,
assigning actual version of application model elements to points of
time.
Note that the type relatedness and root relationships are defined for the
evolution state space as a whole, and are therefore not subject to any
evolution.

In this section we will present a set of wellformedness rules
for application model histories.
These rules represent our {\em way of thinking} with regards to a
wellformed evolution, which is based on strong typing and a strict
notion of identification of instances.
Alternative {\em ways of thinking}, and corresponding wellformedness
rules may be chosen.
For the remainder of this section,
let $H$ be some (fixed) application model history.

\input{gu0601} % Separation of element evolution
\input{gu0602} % Deriving application model versions
\input{gu0603} % Enforcing constraints
\input{gu0604} % An example of element evolution
\input{gu0605} % Evolution of the identification hierarchy
\input{gu0606} % Propagating modifications


==> gu0606.tex <==
\subsection{Propagating modifications}

When an element of the application model evolves (is modified),
other elements may have to be modified
accordingly as these modifications may invalidate others or may 
result in conflicts.
For instance, when the subtyping of object type Medium is terminated
in the LP and CD store running example, all its subtypes must be
terminated as well.
Even more, any relationship type in which such a subtype is involved
must be modified or terminated within the same transaction.

Other dependencies can be found, for example in the context of constraints.
Whenever a new constraint is added, existing instances may be in conflict
with this new rule, and must be adopted to meet the new 
requirements within the same transaction.

These dependencies are enforced on application model histories by
the relations $\IsSch$, $\IsPop$, and $\Depends$,
which require at each point in time the population (at that moment) to be
in accordance with the information structure version (at that moment).
Besides, the information structure version should satisfy the wellformedness
rules of the underlying data modelling technique.




==> hu09.tex <==
\section*{Appendix: PSM Graphical Conventions}
This appendix contains a legenda with the graphical
conventions for object type constructions in PSM
\PostFigure{AppObjTypes}{11.88}
           {Construction mechanisms of PSM}
           {AppObjTypes}


